Visual processing in context of reinforcement learning

Although deep reinforcement learning (RL) has recently enjoyed many successes, its methods are still data inefficient, which makes solving numerous problems prohibitively expensive in terms of data. We aim to remedy this by taking advantage of the rich supervisory signal in unlabeled data for learning state representations. This thesis introduces three different representation learning algorithms that have access to different subsets of the data sources that traditional RL algorithms use: (i) GRICA is inspired by independent component analysis (ICA) and trains a deep neural network to output statistically independent features of the input. GrICA does so by minimizing the mutual information between each feature and the other features. Additionally, GrICA only requires an unsorted collection of environment states. (ii) Latent Representation Prediction (LARP) requires more context: in addition to requiring a state as an input, it also needs the previous state and an action that connects them. This method learns state representations by predicting the representation of the environment's next state given a current state and action. The predictor is used with a graph search algorithm. (iii) RewPred learns a state representation by training a deep neural network to learn a smoothed version of the reward function. The representation is used for preprocessing inputs to deep RL, while the reward predictor is used for reward shaping. This method needs only state-reward pairs from the environment for learning the representation. We discover that every method has their strengths and weaknesses, and conclude from our experiments that including unsupervised representation learning in RL problem-solving pipelines can speed up learning.

==> chaptern_old_deleteme_.tex <==

The previous chapter introduced LARPnets and showed their usefulness in view-point matching experiments in comparison to reinforcement learning methods, in particular model-based ones. The networks learn features that are tailor-made for a prediction module which is then used for graph-based search. This is done in an unsupervised or self-supervised manner and is  independent of a reward function.

However, the method suffers from a higher computational complexity during execution time than model-free methods. Additionally, this method can be extended such that it attempts to reconstruct the salient aspects of the full environment. Namely, the reward function, in addition to the transition function and a possible new state space induced by a learned representation.

With an accurate enough approximation of the environment, we are able to fully train the agent within this reconstructed environment or \textit{world model}. We optimize a policy in a world model defined by our method and show that it compares favorably to the state-of-the-art.

To take advantage of the flexibility gained from learning a model of the environment, we test our agent on varying goals and the representation that the agent learns is a function of not only the observation but also the goal.

The remainder of the chapter has the following structure: We start by discussing related work (Sec.\,\ref{sec:rw}) and covering the basics of reinforcement learning and the MDP optimization problem (Sec.\,\ref{sec:rl}). Then we introduce our world model learning approach, breaking down and explaining each component (Sec.\,\ref{sec:wm}). Next, we show the outer training loop of our method and how model-based and model-free learning is interwoven (Sec.\,\ref{sec:policy}). After that, we construct a suitable environment and show that our method performs competitively compared to state-of-the-art RL methods (Sec.\,\ref{sec:exp}). Finally, we conclude the chapter with a discussion (Sec.\,\ref{sec:disc}).



\subsection{Introduction}

Our model-based LARPnet method is data-efficient and is able to speed to learning for new tasks after pre-training on a similar one. However, model-free reinforcement learning methods have a clear advantage when it comes to the length of the inference time. This is due to the fact that the graph search requires passes to a computationally heavy function to predict future latent states for each potential future step. Depending on the branching factor of the task, this can result in an explosion of computational time. 

In this chapter, we propose to weave together LARPnet with a policy optimization routine to get the best of both worlds from the model-based an model-free reinforcement learning literature, a method we dub Untitled Goal-Condition Policy Learned (UGCPL). 
Since we'll divert our attention to problems with reward signals for this chapter, we expand the network from the previous chapter such that it also has a module for reward prediction. This is conceptually quite simple, as only an additional scalar value needs to be predicted. 

The representation will now also accept a goal vector as an input. This is 
a natural augmentation of the state, as how our perception of the world is influenced by our goals \citep{meltzoff2003imitation}.
This aids in the learning of goal-conditioned policy and allows us to reap the benefit inherent in modeling the environment. 
In the experiments, we show how our training regimen learns a world model which is suitable for the learning of a policy in a model-free manner. This is compared to policies trained from scratch using a model-free methodology and our method beats the baselines in a low-data regime. 


\subsection{Related work} \label{sec:rw}

\textbf{Goal-Conditioned Reinforcement Learning }  Kaelbling studied  environments with multiple goals and small state-spaces in 1993 \citep{kaelbling1993learning}. Their problem setting has an agent with the objective of reaching a known but dynamically changing goal in the fewest number of moves. The observation space was of a low enough dimension for dynamic programming to be satisfactory in their case. Schaul et al's Universal Value Function Approximators \citep{schaul2015universal} tackle environments of larger dimensions by  learning a value function neural network approximator that accepts both the current state and a goal state as the inputs. In a similar vein, Pathak et al. \citep{pathak2018zero} learn a policy that is given a current state and a goal state and outputs an action that bridges the gap between them. 

\textbf{Forward Prediction Dynamics } A popular line of model-based research is learning a forward prediction model of either the full observation space \citep{watter2015embed}, a subset of it \citep{dosovitskiy2016learning} or of learned latent variables associated with the observations \citep{ke2018modeling}. Dosovitskiy et al. \citep{dosovitskiy2016learning} construct a model that predicts a low-dimensional "measurement" subset of the input, which is used for solving environments whose goals are a linear combination of these measurements. A prediction model is generally utilized for planning \citep{hlynsson2020latent, silver2017predictron} when modeling the reward is not feasible.

\textbf{World Models } Other methods incorporate a prediction model into a full replica of the environment which can be used for a simulated optimization of the agent. The seminal "world model" algorithm is Sutton's 1991 Dyna architecture \citep{sutton1991dyna} where an agent is described that models the environment dynamics and receives rewards from simulated experience in addition to real-world experience. Ha and Schmidhuber \citep{ha2018world} use a similar algorithm where the state representation is learned in an unsupervised manner. Other twists on the Dyna policy-learning scheme include  SimPLE \citep{kaiser2019model}, MuZero \citep{schrittwieser2019mastering} and DreamerV2 \citep{hafner2020mastering}. 
%More goal-c. RL: https://arxiv.org/pdf/1911.08453.pdf, https://arxiv.org/pdf/1802.09081.pdf, https://arxiv.org/pdf/1811.11359.pdf, https://arxiv.org/pdf/2004.08356.pdf, https://arxiv.org/pdf/1612.08810.pdf

% schmidhuber2015learning <- iteratively learns a world model and controller

% \textbf{Learning within world models} 

The method we propose in this chapter can be categorized as a hybrid model-based / model-free method, as it learns first a model of the environment that is then used for model-free learning.%https://www.repository.cam.ac.uk/bitstream/handle/1810/298048/thesis.pdf?sequence=1&isAllowed=y

\subsection{Learning the World Model} \label{sec:wm}

In this section, the representation-learning aspect of the module is described. The novel contribution is the goal-dependency of the representations, in addition to being directly learned for the useful downstream tasks of predicting rewards and latent representations. The module as a whole is first described before each component is explained in turn.

\subsubsection{Module Outline}



The representation learning module is made up of the following components (Fig~\ref{fig:boat1}): 

\begin{figure}[ht!]
  \begin{center}
        \includegraphics[width=0.8\linewidth]{assets/beedance_b.pdf}
  \caption[Illustration: Representation Learning Module]{\textbf{Representation Learning Module }  The module is comprised of representation, reward prediction and representation prediction units. Each batch contains: the observations at time steps $t$, $t+1$ and $n$, where $n$ is a random sample from the buffer, the action taken at time $t$ and the agent's internal goal at time $t$.}
  \label{fig:boat1}
  \end{center}
\end{figure}

\begin{enumerate}
  \item Inputs
    \begin{itemize}
     \item The goal (fixed per rollout)
     \item The observations at time steps $t$, $t+1$ and $n$ (see triplet loss section)
     \item The action at time step $t$
     \item The reward at time step $t+1$
   \end{itemize}
  \item Functions with learnable parameters
    \begin{itemize}
     \item The representation
     \item The reward predictor
     \item The latent representation predictor
   \end{itemize}
   \item Loss functions
    \begin{itemize}
     \item Triplet loss between representations
     \item Mean-squared error (MSE) loss for the reward predictor
     \item MSE loss for the representation predictor
   \end{itemize}
\end{enumerate}



Since the module is fully differentiable, every component is optimized in an end-to-end manner during the world-model update step (see below). We don't assume a useful metric or natural ordering  between the goals and action so the goal and action inputs are converted from integers to one-hot encodings.

\subsubsection{Triplet Loss}


Of the methods considered for alleviating the problem of trivial solutions in the previous chapter, we chose the triplet loss (Fig. \ref{fig:boat6}) due to being potentially more stable than whitening and requiring fewer parameters than a reconstructive loss.

\begin{figure}[ht!]
  \begin{center}
  \includegraphics[width=.65\linewidth]{assets/triplet_loss_worldmodel.pdf}
  \caption[Illustration: Triplet Loss]{\textbf{Triplet Loss } Three copies of the representation network each receives an observation and the goal from that observation's rollout. The negative is a random observation from the buffer that is not in $\{t-1, \dots, t+2\}$ from the same rollout. }
  \label{fig:boat6}
  \end{center}
\end{figure}    

The triplet loss function has the form

$$\mathcal{L}(A, P, N) =   \max({ d_{+} -  d_{-}+{m}, 0})$$

where $m$ is the margin and the positive and negative distances are defined as

$$ d_{+} = ||  \phi(A) - \phi(P)||^2$$

$$ d_{-} = ||  \phi(A) - \phi(N)||^2$$

and $\phi$ is the representation.



\subsubsection{Predicting the Next-step Reward and Latent Representation}

The representation and action at time step $t$ is simultaneously passed to two separate functions (Fig.~\ref{fig:boat7}) that predict the next-step reward and representation. Both have simple mean-squared error losses. The reward prediction network will be used to approximate the reward function in the world model and the representation prediction network approximates the transition function. 
\clearpage
\begin{figure}[ht!]
\begin{center}

  \includegraphics[width=.75
  \linewidth]{assets/predrew_loss_worldmodel2.pdf}
  \caption[Illustration: Prediction Losses]{\textbf{Prediction Losses}. Both networks receive the same inputs and are trained at once in each training step. They are drawn here with dense layers but they can in principle be any differentiable function.}
  \label{fig:boat7}
  \end{center}

\end{figure}



\subsection{Learning the Policy} \label{sec:policy}

\subsubsection{Train Time}

To ensure that the world model is modeling the facets of the environment that are of the most value to the agent, we do an iterative training of the world model and the policy (Alg.~\ref{alg:wm}). The (initially random) policy $\pi$ is used to gather training data in the MDP $\varepsilon_T = (\mathcal{S}, \mathcal{A}, \mathcal{P}, \mathcal{R}, \mathbb{P}(s_0), \lambda)$ for the representation $\phi$, reward predictor $\zeta$ and representation predictor $\xi$. We use the functions that make up our world model, the representation $\phi(\mathcal{S})$, the reward function is $\zeta = \hat{\mathcal{R}}$ and the transition function $\xi = \hat{\mathcal{P}}$, to create a new MDP: $\varepsilon_F = (\phi(\mathcal{S}), \mathcal{A}, \zeta, \xi, \mathbb{P}(s_0), \lambda)$. The policy is trained inside the new environment $\varepsilon_F$ and then used to gather more data again to train the world model further.

% Inspiration for similar algos: 
% https://www.cs.toronto.edu/~vmnih/docs/dqn.pdf
% https://arxiv.org/pdf/1903.00374.pdf
% https://arxiv.org/pdf/1803.10122.pdf
% https://arxiv.org/pdf/1801.06176.pdf
\begin{algorithm}[H]
\SetAlgoLined
 Initialize environment $\varepsilon_T$\;
 Initialize policy $\pi$\;
 Initialize representation $\phi$, reward predictor $\zeta$ and representation predictor $\xi$\;
 Initialize experience buffer $B$\;
 \While{not done}{
  Perform rollout using $\pi$ and append the states, actions and rewards to $B$\;
  Duplicate the terminal state, action reward tuples $\kappa$ times to help balance the data set\;
  \If{world model update step}{
     Train $\phi$, $\zeta$, and $\xi$ on the buffer $B$\;
   }
  \If{policy update step}{
   Assemble environment $\varepsilon_F$ with $\phi$, $\zeta$, and $\xi$\;
   Train $\pi$ on $\varepsilon_F$ for $T$ time steps\;
   }
   Shuffle B and keep the first $N$ experiences\;
 }
 \caption{Training of World Model and Policy}
 \label{alg:wm}
\end{algorithm}





\subsubsection{Inference Time}

When the world model and policy have been trained, the representation $\phi$ is extracted from the module. At each time step $t$, the observation $O_t$ and the goal vector $G$ are passed to $\phi$ (Fig. \ref{fig:boat5}) which yields the latent-space vector. This vector is passed to the policy $\pi$ which outputs the estimated optimal action $a_t$ which is passed to the environment, yielding $O_{t+1}$ and so on.

\begin{figure}[ht]
\begin{center}

  \includegraphics[width=.7\linewidth]{assets/action_pipeline.pdf}
  \caption[Illustration: Policy at Inference Time]{\textbf{Policy at Inference Time} The test time procedure is the same as for regular model-free reinforcement learning, except that the input to the policy is the latent vector given by the representation from the observation as well as the environment's goal parameter. }
  \label{fig:boat5}
\end{center}
\end{figure}



\subsection{Experiments} \label{sec:exp}
In this section, we evaluate our method on a simple but dynamic navigation environment. In \ref{subsec:env} the environment we created for the experiments is introduced. In  \ref{subsec:cm} we discuss the baseline methods that we compare our method to. Sec. \ref{subs:ma} contains the details of our model parameters. In Sec. \ref{subsec:policy} we describe the parameter values of Alg. \ref{alg:wm}. Finally, Sec. \ref{subsec:results} outlines the results of the experiments. 

\subsubsection{Environment} \label{subsec:env}

The method is tested in a four-room gridworld environment based on the Minimalistic Gridworld Environment (MiniGrid) \citep{gym_minigrid} (Fig.~\ref{fig:boat4}). The world is a $8 \times 17$ grid of tiles, split into two rooms, with each tile containing one or zero objects. 

The environment fits naturally into our MDP tuple template $(\mathcal{S}, \mathcal{A}, \mathcal{P}, \mathcal{R}, \mathbb{P}(s_0), \lambda)$: 
\begin{itemize}
    \item[$\mathcal{S}$:]The constituent states of $\mathcal{S}$ are determined by the agent's location (which tile it occupies) and direction (facing north, west, south or east) along with the goal's location. The steps taken since the initialization of the run and the maximum number of steps until timeout also matter for the calculation of the reward.
    \item[$\mathcal{A}$:]The action space $\mathcal{A}$ consists of three action: (1) turn left, (2) turn right and (3) move forward.
    \item[$\mathcal{P}$:] Each action brings about the indicated change to the state, making $\mathcal{P}$ a deterministic function.
    \item[$\mathcal{R}$:] Reaching the green tile goal gives a reward of $1 - 0.9 \cdot \frac{\# \textrm{steps taken} }{\# \textrm {max step}}/ $, every other action gives 0 points. The environment automatically times out after 1000 steps.
    \item[$\mathbb{P}(s_0)$:] the agent is placed between two of the rooms facing a random direction and has to go to either one of two goal locations (Fig.~\ref{fig:boat4}).
    \item[$\lambda$:] the discount factor is set to $0.99$ for the purpose of all model-free policy training routines
    
\end{itemize}

   The agent's observation is comprised of its field of vision -- a 28x28 pixel rgb array -- as well as a categorical variable describing the agent's goal.
 
% \begin{figure}[h]
%   \includegraphics[width=.5\linewidth]{assets/top_goal.png}
%   \caption{First goal}
%   \label{fig:boat3}
%     \includegraphics[width=.5\linewidth]{assets/bottom_goal.png}
%   \caption{Second goal}
%   \label{fig:boat4}
% \end{figure}

\begin{figure}[!tbp]
  \centering
  \begin{minipage}[b]{0.6\textwidth}
    \includegraphics[width=\textwidth]{assets/top_goal.png}
    % \caption*{(a)}
        \includegraphics[width=\textwidth]{assets/bottom_goal.png}
  \end{minipage}
%   \hfill
%   \begin{minipage}[b]{0.4\textwidth}
%     \includegraphics[width=\textwidth]{assets/bottom_goal.png}
%     \caption*{(b)}
%   \end{minipage}
  \caption[Example: The Room Environment]{\textbf{The Room Environment } The goal locations are indicated by the green square and the run is a success when the red agent reaches it. The light gray areas are impassable walls. Each row shows a snapshot of a different state.  The left side shows the full state of the environment and the right side shows the observations emitted by the environment.}
 \label{fig:boat4}

\end{figure}


\subsubsection{Baselines} \label{subsec:cm}
 We compare our method to canonical, state-of-the-art reinforcement learning algorithms: 

\begin{itemize}
    \item 
For initial sanity-checks, we measure the performance of a purely \textbf{random policy} on the environment.
\item Actor Critic using Kronecker-Factored Trust Region (\textbf{ACKTR}) \citep{wu2017scalable}, which combines actor-critic methods, trust-region optimization and distributed Kronecker factorization to enhance sample-efficiency. 
\item A version of Proximal Policy Optimization (\textbf{PPO2}) \citep{schulman2017proximal}. It modifies the original PPO algorithm by using clipped value functions and a normalized advantage.
\end{itemize}


The comparison algorithms are implemented by Stable Baselines \citep{stable-baselines} 
and we use all the default parameters of the methods. 

This includes the so-called Nature CNN architecture used for the model. This model is orders of magnitude larger than our method \ref{tab:totalparams} so we also construct a smaller version of it, see the next section for details. 

\subsubsection{ Model Architectures} \label{subs:ma}

Every policy and predictor is realized as a neural network using Keras \citep{chollet2015keras}.  We will describe here precisely the architecture used for each model and refer to tables in the appendix for better visualizations.

\textbf{Our representation network} is a convolutional network (Table \ref{tab:repnet})  with a $56 \times 56 \times 5$ input consisting of the raw $56 \times 56 \times 3$ visual observation stacked with the one-hot  $56 \times 56 \times 2$ plane indicating the goal. The first layer subsamples the input, keeping only every other column and row. This is followed by 8 filters of size $3 \times 3$ with a stride of 3 and no padding. This is followed with a ReLU activation and a $2 \times 2 $ pooling layer with a stride value of 2. The pooling layer's output is passed to a layer with 16 convolutional filters of size $3 \times 3$ and a stride of 2 and a ReLU activation function. The output is then flattened and passed to a dense layer with 16 units and a linear activation, defining the dimension of the representation. To allow us to fix the margin of the triplet loss, we fix the scale of the features by performing an L2-normalization in the last layer:

$$ \textbf{x} \leftarrow \frac{\textbf{x}}{\sqrt{\sum_{i=1}^dx^2_i}} $$

\textbf{Our policy network} is a three-layer fully-connected network (Table \ref{tab:polnet1}) accepting the 16 dimensional representation as input. The first two layers have 64 units and a ReLU activation and the last layer has 3 units and a linear activation function. 

\textbf{Our latent representation prediction network} is a four-layer fully-connected network (Table \ref{tab:polnet2}) accepting the 16 dimensional representation concatenated with the 3 dimensional one-hot representation of the action as input. The first two layers have 512 units and ReLU activations, followed by a 256 unit layer with a ReLU activation and the last layer has 16 units and a linear activation. 

\textbf{Our reward prediction network} is a three-layer fully-connected network (Table \ref{tab:polnet3}) with the same input as the latent representation prediction network. The first two layers have 256 units and a ReLU activation but the last layer has 1 unit and a logistic activation function. 


\textbf{The comparison policy network} is the original DQN \citep{mnih2013playing}. The input is the same as for the representation network. The first three hidden layers are convolutional layers: the first has 16 $8 \times 8$ filters with stride 4, the second has 32 filters of size $4 \times 4$ with stride 3 and the third has 32 filters of size $3 \time 3$ with stride 2. The final hidden layer is a fully-connected layer with 256 units and the output layer is a fully-connected linear layer with 3 units, one for each action. Each hidden layer has a ReLU nonlinearity. We also built a smaller version of the net to bring the parameter count closer to our method, which is the same except with a fourth of the number of convolutional filters and eight of the number of units in the hidden dense layer.

\subsubsection{Training the policy} \label{subsec:policy}

Here we fill in the details of Alg.\,\ref{alg:wm}.  The policy is the fully-connected network described above, trained using PPO2.

The functions  $\phi$, $\zeta$ and $\xi$ are already described above. The experience buffer has a capacity of $N = 30k$. We oversample states-action pairs that result in a positive reward $\kappa=300$ times. This number was determined by experiments to be sufficient to balance the data set, resulting in roughly a third of it containing positive rewards. 

The while loop ends after 200 iterations and each rollout consists of 500 steps. The full world model is trained for the first 50 iterations, after which the representation $\phi$ stops receiving updates. The policy is likewise updated for 500 steps in the world model $\varepsilon_F$ in every iteration. 

\subsubsection{Results} \label{subsec:results}

% TODO: Make each room smaller and add two additional rooms ... try 6x6 rooms or so

%TODO: See if I rather want my goal input to enter later, a lá http://proceedings.mlr.press/v37/schaul15.pdf Fig. 1

%TODO: Test my environment on fully-observable environment where I pass in the goal state and see how it generalizes to new goals.

%TODO: Try different encodings for goals (location with a fully observable environment)

% TODO: Try a heatmap of visited areas

%TODO: Finish the discussion section

% TODO: Add a table with aggregate results from the graphs

% TODO: Log more noteworthy data: "computational budget", "training time"

% TODO: Add a visualization a lá http://proceedings.mlr.press/v37/schaul15.pdf Fig. 4, Fig. 2, Fig. 8, 

%( TODO: Add graphic for the inverse loss)
\textbf{Qualitative Analysis } 
% 140 + [untracked: ] 0

We visualize the structure in our environment as perceived by our agent in Fig.\,\ref{clusterings}.   We condition the representation on the two different goal locations and find no qualitative difference. Notice how the embeddings contain a meaningful cluster of states with a wall on the right-hand side in the upper right (orange and red dots), states with a wall on the left-hand side in the bottom left (blue and purple dots) with the states surround the door in the middle (earth-colored dots).

\begin{figure*}[ht]
	\centering
	\begin{minipage}{.27\columnwidth}
		\centering
	\includegraphics[width=\textwidth]{assets/env_groundtruths.pdf}
		\label{label1}
	\end{minipage}%
	\begin{minipage}{.36\columnwidth}
		\centering
	\includegraphics[width=\textwidth]{assets/0_0_env_groundtruths.pdf}
	\end{minipage}
\begin{minipage}{.36\columnwidth}
		\centering
	\includegraphics[width=\textwidth]{assets/0_1_env_groundtruths.pdf}
	\end{minipage}
		\caption[Result: Representation Clustering]{ \textbf{Representation Clustering } We use t-SNE \citep{maaten2008visualizing} to visualize the topology of our 16-dimensional embeddings of the environment states as the agent faces north.}
		\label{clusterings}
\end{figure*}

\textbf{Baselines } A policy that takes random actions only gets an average cumulative reward of around $0.3$, which is added to each following graph as a horizontal line. The results for ACKTR using the two different Nature CNNs are displayed in Fig.\,\ref{acktr}. There is not a noticeable difference between the larger and the smaller networks on the scale of the data that we're using. On the other hand, PPO2 performs reaches much lower reward values and is more unstable than ACKTR. (Fig.\,\ref{ppo2results}).  


\begin{figure*}[ht]
	\centering
	\begin{minipage}{.45\columnwidth}
		\centering
		\includegraphics[width=\textwidth]{assets/acktr_nature.png}
		\label{label1a}
	\end{minipage}%
	\hspace{-1em}
	\begin{minipage}{.45\columnwidth}
		\centering
		\includegraphics[width=\textwidth]{assets/acktr_smaller.png}
		\label{label2a}
	\end{minipage}
		\caption[Result: ACKTR Training]{ \textbf{ACKTR training results.} In each run, 10 test rollouts are performed and the mean cumulative reward is averaged.}
		\label{acktr}
\end{figure*}


\begin{figure*}[ht]
	\centering

	\begin{minipage}{.49\columnwidth}
		\centering
		\includegraphics[width=\textwidth]{assets/ppo2_big.png}
	\end{minipage}%
	\hspace{-0.45em}
	\begin{minipage}{.49\columnwidth}
		\centering
		\includegraphics[width=\textwidth]{assets/ppo2_small.png}
	\end{minipage}
		\caption[Result: PPO2 Training]{ \textbf{PPO2 training results.} The agents are considerably less stable and worse performing than ACKTR and ours. }
		\label{ppo2results}
\end{figure*}


\textbf{Only Pre-trained World Models } We initially organize the training of our method in a manner akin to Ha and Schmidhuber's policy learning \citep{ha2018world}: the world model is initially trained on 75 thousand random steps, after which the policy is trained and no further updates to the world model are made. 
The training curve for this setup is in Fig.\,\ref{graph:75k}.
We then vary the number of pretraining steps and present the results for 30k, 10k and 1k random initial interactions to gather data for the world models.  (Fig.\,\ref{fig:varying}). The case with no world model training steps at all was also considered (Fig.\,\ref{fig:varying}, bottom right), where the agent's performance is quickly pushed to 0.
More pre-training steps are better and at least 10k steps are sufficient for training inside of the world model to significantly outperform the random baseline. 
Unsurprisingly, training the policy within an untrained world model does not improve the policy's performance in the real-world environment


\begin{figure}[ht]
\begin{center}
  \includegraphics[width=.65\linewidth]{assets/ownmeth2.png}
  \caption[Result: Own Method after Pre-training.]{\textbf{Own Method after Pre-training.} Own method was pre-trained on 75k steps,  aggregated over 3 agents with 10 test rollouts each. The error bands indicate one standard deviation from the mean.}
  \label{graph:75k}
\end{center}
\end{figure}
\begin{figure}[htp]
\centering
\includegraphics[width=.4\textwidth]{assets/ownmeth_30k.png}
\includegraphics[width=.4\textwidth]{assets/ownmeth_10k.png}
\includegraphics[width=.4\textwidth]{assets/ownmeth_1k.png}
\includegraphics[width=.4\textwidth]{assets/ownmeth_0k2.png}
\caption[Result: Our Method with Varying Initial data Collection Lengths]{\textbf{Our method with Varying Initial data Collection Lengths.}}
\label{fig:varying}
\end{figure}

\textbf{Iterative updates } 
Following our full iterative world-model / policy optimization scheme from  Alg.\,\ref{alg:wm} yields the results in Fig.\,\ref{ouriterative}. 
This looks a little better and more stable than the versions with pre-training only. Even though our method is equipped with fewer parameters, it reaches better performance than the baselines Rl methods. Our iterative training regime is also more stable and reaches good performance quickly. 

\begin{figure*}[ht]
	\centering
	\begin{minipage}{.65\columnwidth}
		\centering
		\includegraphics[width=\textwidth]{assets/rlyonthego_longer.png}
	\end{minipage}
		\caption[Result: Our Method with Iterative Optimization]{ \textbf{Our method with Iterative Optimization.} The policy is not tested until it has been trained 2k times.}
		\label{ouriterative}
\end{figure*}


\textbf{Inverse Model Normalization } 
We considered omitting the triplet loss in the hope that predicting the reward alone is sufficient for learning informative representations. However, due to the sparse-reward nature of our experiments, we found that this resulted in the system learning a representation that is constant over state-goal pairs that do not result in a reward (maximizing latent  predictability) but changing only when the next step will yield a reward (maximizing  reward predictability). This is not helpful for approximating the environment dynamics. 

Instead of relying on the triplet loss, we also try exchanging it with an inverse model loss. By inverse model, we mean that we add a predictive network to our training module for predicting $a_t$ given $\phi_t$ and $\phi_{t+1}$. The motivation for this is that the change in the representation should be informative enough for the action to be recoverable again, which could substitude the triplet loss for preventing trivial solutions \citep{pathak2017curiosity}. The model for the inverse predictor is identical to the one for the reward prediction, except that the output layer has 3 units and a softmax activation. The results for this setup are shown in Fig.\,\ref{inversedyn}.

\begin{figure*}[ht]
	\centering
	\begin{minipage}{.7\columnwidth}
		\centering
		\includegraphics[width=\textwidth]{assets/inversedyn.png}
	\end{minipage}
		\caption[Result: Our Method with  Inverse Model Regularization]{ \textbf{Our Method with Iterative Optimizations and Inverse Model Regularization.}}
		\label{inversedyn}
\end{figure*}

\textbf{Inference Time Length } We measured the time it took for UGCPL to choose an action, compared
to LARPnets and the baseline RL models. The benchmarks were made on a machine with an Intel(R) Xeon(R) CPU E5-1650 v4 @ 3.60GHz CPU, a Tesla P40 and a GeForce GT 710 GPUs.  
The LARPnets 162 states before returning the action to take, explaining the vast difference in the execution time between the LARPnets and the others. 
The Intel processor has 2 threads per core and 6 cores per socket, totaling in 12 CPUs. This explains the discrepancy in the wall-clock time and CPU time for some of the algorithms, as up to twelve processors were performing computations for the process. 
\begin{table}[ht]
    \centering \begin{tabular}{|l c c|} 
     \hline\rule{0pt}{2.2ex}
     \textbf{Method} & \textbf{Wall-Clock Time (ms)} & \textbf{CPU Time (ms)} \\ [0.5ex] 
     \hline\rule{0pt}{2.2ex}UGCPL & 921.7 $\pm$ 97.9 & 1716.0 $\pm$ 119.8 \ \ \\[.5ex] 
      LARPnets & 389,351.5 $\pm$ 17,807.28 & 663,413.0 $\pm$ 29,721.6 \ \  \\[.5ex]
      %LARPnets & 34239.1e-5 $\pm$ 4173.8e-5 & 54510.7e-5 $\pm$ 4944.3e-5  \\[.5ex]
      PPO2, Larger & 22.4 $\pm$ 1.6 & 22.9 $\pm$ 1.4 \\[.5ex]
      PPO2, Smaller & 24.3 $\pm$ 0.5 & 23.9 $\pm$ 0.5\\[.5ex]
      ACKTR, Larger & 24.1 $\pm$ 1.2 & 
23.6 $\pm$ 1.5 \\[.5ex]
      ACKTR, Smaller & 25.0 $\pm$ 0.4 &
24.5 $\pm$ 0.7 \\[.5ex]
    \hline
    \end{tabular}
    \vspace{0.1cm}
    \caption[Result: A Comparison of Execution Times]{A Comparison of Execution Times.}
    \label{tab:inference_times}
\end{table}





\subsection{Discussion and Future Work} \label{sec:disc}


In this chapter, we put forward Untitled Goal-Conditioned Policy Leaner (UGCPL), a hybrid model-based model-free reinforcement learning method for environments with varying goals. Initial experiments indicate that our method learns faster and is more stable than proven model-free RL methods that have similarly sized models. 

Future work for this chapter includes:

\begin{itemize}
    \item Add two rooms to the left and reduce the room sizes to $5 \times 5$ or $6 \times 6$
    \item Add experiments where we add the goal representation rather as an input to the reward prediction and latent representation prediction functions
    \item Try different forms of the goal inputs: \begin{itemize}
        \item location coordinates
        \item goal state (as full observation)
    \end{itemize} In the case of a goal state, changing the environment to be fully observable would be preferable. Both options open up the possibility of generalizing to unseen goal locations.
    \item Add more visualizations: \begin{itemize}
        \item a heatmap of most visited states during test rollouts
        \item most taken actions at each location
        \item policy values at each state
    \end{itemize} 
    \item Add a table or tables summarizing and aggregating the most interesting statistics in our policy training curves

\end{itemize}

Future work for the thesis as a whole includes:
\begin{itemize}
\item Add a chapter or a section where the main unsupervised learning methods (e.g. pca, sfa, t-sne, vaes, umap, lda, gda)  are combined with model-based reinforcement  learning. This will help bridge together the representation-focused early chapters of the thesis with the reinforcement-learning focused later chapters.
\end{itemize}


==> measuring_chapter.tex <==

In this paper, we propose a new experimental protocol and use it to benchmark the data efficiency --- performance as a function of training set size --- of two deep learning algorithms, convolutional neural networks (CNNs) and hierarchical information-preserving graph-based slow feature analysis (HiGSFA), for tasks in classification and transfer learning scenarios. The algorithms are trained on different-sized subsets of the MNIST and Omniglot data sets. HiGSFA outperforms standard CNN networks when the models are trained on 50 and 200 samples per class for MNIST classification. In other cases, the CNNs perform better. The results suggest that there are cases where greedy, locally optimal bottom-up learning is equally or more powerful than global gradient-based learning.

The remainder of the chapter is structured as follows: the importance of data-efficiency in the context of learning is emphasized, especially compared to the learning capabilities of human beings in Section~\ref{sec:measuring_introduction}. The most relevant related work is discussed in Section~\ref{measuring_relatedwork}. Our experimental framework is described in Section~\ref{measuring_relatedwork} and we give technical details of the algorithms that we compare in this work. The results of our experiments are outlined in Section~\ref{measuring_results} and we close the chapter with a discussion of our findings in Section~\ref{measuring_discussion}.

\section{Introduction}
\label{sec:measuring_introduction}

\noindent In recent years, we have seen convolutional neural networks (CNN) dominate benchmark after benchmark for computer vision since the 2012 ImageNet competition breakthrough \citep{krizhevsky2012imagenet}. These methods prosper with an abundance of labeled data, and an abundance of data is often required for acceptable results \citep{oquab2014learning}. In contrast, for most people, it is only necessary to see one picture of an Atlantic Puffin to be able to identify correctly such a bird as one. \\
\indent To be fair, we have a lot of prior experience. It is easy to make a mental note: ``a puffin is a small black and white bird with orange feet and a colorful beak'' because we have learned a useful representation of the salient aspects of the image. Instead of being bogged down by the details of every exact pixel value, as an untrained AI might, we can focus our attention on the most useful features of the image. \\
\indent For this reason, investigations on the efficacy of methods to learn a concept from few samples are often done through the lens of representation learning \citep{bengio2013representation}, for example via transfer learning \citep{pan2010survey} or low-shot learning \citep{wang2018low}. \\
\indent In this work we consider a method to measure data efficiency, the performance of an algorithm as a function of the number of data points available during training time, which is an important aspect of machine learning \citep{kamthe2017data},  \citep{al2015efficient}. We quantitatively examine the performance of CNNs and hierarchical information-preserving graph-based slow feature analysis (HiGSFA) \citep{escalante2016improved} networks for varying training set sizes and for varying task types. \\
 \indent HiGSFA has been chosen because it is the most recent supervised extensions of slow feature analysis (SFA) and has shown promise in visual processing with a notable distinction from CNNs: the computation layers are trained in a "greedy" layer-wise manner instead of via gradient descent \citep{escalante2016improved}. \\
 \indent The methods are applied to  visual tasks: a simple version of the MNIST classification task, where we vary the number of training points, and increasingly difficult tasks constructed from the Omniglot data set. Our \textbf{contribution} in this work is a novel experimental protocol for evaluation of transfer learning applied to experimentally evaluate CNNs with the slowness-based HiGSFA.

\section{Related Work}
\label{measuring_relatedwork}
\noindent Gathering data can be quite costly, so the question "how much is enough" has been considered in literature ranging from classical statistics \citep{krishnaiah1980handbook} over pattern recognition \citep{raudys1991small} to experimental design \citep{beleites2013sample}.
As data plays a central role in machine learning as well, the study of its effective use has garnered attention from all branches of the field. \\
\indent In a similar vein as our work, \citep{lawrence1998size} analyze the effect of generalization when the number of sample points are varied for supervised learning tasks. Equipped with the prior that supervised learning methods' performance obeys the inverse power law, \citep{figueroa2012predicting} trained a model to predict the classification accuracy of a model given a number of inputs.\\
\indent Transfer learning straddles the intersection between supervised learning and unsupervised learning, where the focus is uncovering representations that are both general and also useful for particular applications. The  Omniglot data set we consider was introduced in \citep{lake2015human} and has been popular  for developing transfer learning methods \citep{bertinetto2016learning}, \citep{edwards2016towards}, \citep{schwarz2018progress}.\\ 
\indent
With its sparse rewards and problems of credit assignment, reinforcement learning (RL) has a particular need for data efficiency, motivating such early works as prioritized sweeping \citep{moore1993prioritized}. More recently, \citep{riedmiller2005neural} designed the neural-fitted Q-learner for data efficiency. This method has been successfully combined with deep auto-encoder representations for visual RL \citep{lange2010deep}. Deep Q-Networks have made better still use of data for RL by combining experience replay, target networks, reward clipping and frame skipping \citep{mnih2013playing} \citep{mnih2015human}.\\
\indent
SFA was introduced in 2002 by Wiskott and Sejnowski as an unsupervised learning method of temporally invariant features \citep{wiskott2002slow}. These features can be learned hierarchically in a bottom-up manner, reminiscent of deep CNNs: slow features are learned on spatial patches of the input and then passed to another layer for slow feature learning.  The method is then called hierarchical slow feature analysis (HSFA) and has attracted attention in neuroscience for plausible modeling of grid, place, spatial-view, and head-direction cells  \citep{franzius2007slowness}. \\
\indent For labeled data, the method admits a supervised extension in the form of graph-based SFA (GSFA)  \citep{escalante2013solve}. Information is often lost in early layers of hierarchical SFA --- that could contribute to a globally slower signal --- prompting the development of HiGSFA  \citep{escalante2016improved}.\\
\indent Deep learning extensions of SFA is currently an active research area. The SFA problem is  solved with stochastic optimization in Power-SFA  \citep{schuler2018gradient}. A differentiable whitening layer is constructed, allowing for a non-linear expansion of the input to be learned with backpropagation. Another recent method, SPIN \citep{DBLP:journals/corr/abs-1806-02215} learns eigenfunctions of linear operators with deep learning methods and can be applied to the SFA problem as well.

\section{Methods}


\noindent Below we describe the novel experimental setup as well as the methods being evaluated using the setup. For the remainder of the article we assume CNNs to be well-known and understood but we can recommend  \citep{cs231n2017convolutional} as a good pedagogical introduction to the method.

\subsection{HiGSFA}


HiGSFA belongs to a class of methods motivated by the slowness principle, which is based on the assumption that important aspects vary more slowly than unimportant ones \citep{sun2014dl}. This model takes as input data points such that data point $x_n$ is node $n$   in an undirected graph with weight $v(n)$. This can control the relative weight each data point has during the training but we set it as uniformly 1 is our experiments below.


The edge between nodes $n$ and $n'$ is $\gamma_{n, n'}$ and signifies a relationship between the data. This could be their spatial or temporal proximities or whether they belong to the same class.

For instance, during our classification tasks below,  we set:

\begin{equation}
    \gamma_{n, n'}= 
\begin{cases}
    1,& \text{if } n \text{ and } n' \text{ in same class}\\
    0,              & \text{otherwise}
\end{cases}
\end{equation}

Given a function space $\mathcal{F}$ with elements $g_j$, we learn slowly varying features $y_j(n) = g_j(x_n)$ of the data by solving the optimization problem \citep{escalante2013solve}:


\begin{equation}
\begin{aligned}
& \underset{g_j}{\text{minimize}}
& & \frac{1}{R} \gamma_{n, n'} \sum\limits_{n, n'} \left( y_j(n) - y_j(n') \right)^2 \\
& \text{subject to}
& & \frac{1}{Q} \sum\limits_{n} v_n y_j(n)\ \  \ \ \ \ \ \, = 0   \ \ \ \ \ \ \ \ \ \,  \\
&&& \frac{1}{Q} \sum\limits_{n} v_n \left(y_j(n) \right)^2\, \ \ \ = 1  \ \ \ \ \ \ \ \ \ \ \, \\
&&& \frac{1}{Q} \sum\limits_{n} v_n y_j(n) y_{j'}(n) = 0\text{, } j' < j \ \\
& \text{where}
&&Q = \sum\limits_{n}     v_n,\ R = \sum\limits_{n, n'} \gamma_{n, n'}
\end{aligned}
\end{equation}

The first constraint secures weighted zero mean, the second constraint secures weighted unit variance and the third one secures weighted decorrelation and order. \\
\indent To reduce computational complexity, we extract features of the data hierarchically. Similarly to CNNs, we extract features from $F \times F$ patches of the image data in the first layer, then extract features of $F' \times F'$ patches of the output features in the next layer and so on. The layers are trained by solving the optimization problem, one layer at a time, from the input layer to the output layer. The layer-wise parameters can be shared.


As we can experience information-loss while doing these layer-wise optimizations, an information-preserving mechanism is added. The cost function is minimized locally, so we can experience information-loss if dimensions are discarded that do not minimize the function on a local level --- but could conceivably be better for the overall problem.

For each layer (figure \ref{example}), a threshold is placed on the features with respect to their slowness. If an output feature or features would be too fast, we replace them by the most variance-preserving PCA features. Each layer thus outputs a combination of slow features and PCA features.

\begin{figure}[ht]
  %\vspace{-0.2cm}
  \fontsize{31}{05}\selectfont
  \centering
   {\resizebox*{0.4 \textwidth}{!}{\includegraphics
    {files/graphic.PNG}}}
  \caption[Illustration: HiGSFA Network Layer]{\textbf{HiGSFA Network Layer.} The feature generation is similar to that of the CNN. The layer outputs $N$ channels of slow features and $M$ channels of PCA features. The number of PCA channels features is either fixed beforehand or determined by replacing a number $M$ of the SFA features whose \textit{slowness} (cost function in eq. 2) exceeds a given threshold.}
  \label{example}
 \end{figure}
 
 \subsection{General description of protocol}

The performance of two hypothesis $h_1$ and $h_2$, not necessarily from the same hypothesis set $\mathcal{H}$, is compared on a classification task. The learning curves of the two hypothesis are plotted as a function of the number of data points in the training set. This can be done simply by taking an increasing number of training points per class as we evaluate using MNIST, below. \\
\indent Alternatively, the number of training points per class are kept constant and the number of classes are varied. The relationship training and test set distributions is also altered, such that the task ranges from classical classification to transfer learning. We report a comparison of methods below using this scheme on the Omniglot data set. 



\subsection{Evaluation on MNIST}
First, we compare classification accuracies on MNIST  \citep{lecun1998gradient} as a function of the number of samples per class used during training. The images have a dimension of $28 \times 28$ pixels.  For 100 iterations, we choose random samples from each class and use a thousand unused samples from each class for validation. Finally, the models are tested on the classic 10 thousand test images.

\subsection{Architectures}

We constructed a two-layer HiGSFA network with circa 13k parameters (the number is stochastic and changes from training set to training set), extracting 400 features from the data. The first layer has a filter size of $5\times5$ and a stride of 2, extracting 25 features for each spatial patch. The second layer has a filter size of $4\times4$ and a stride of 2, extracting 16 features for each spatial patch. \\
\indent The output of the first layer is concatenated with a copy of itself, where each element $x$ is replaced with $|x|^{0.8}$, doubling the number of channels and giving us nonlinearity.  If the value of the objective function is larger than a threshold of 1.99, we select PCA features. This upper bound is motivated by the fact that non-predictive, white noise features take a value of 2 in the objective function \citep{creutzig2008predictive}. The parameters within each layer are shared. A single-layer softmax neural network was trained on the features of the second layer to handle classification, which has 4010 parameters.\\
\indent Two standard CNNs were constructed as well, one with the constraint to have a similar number of parameters as the HiGSFA network, and another with an amount closer to what is seen in practice on similar data sets. That is to say, the smaller CNN corresponds to the HiGSFA network. \\
\indent We call the smaller network CNN-1 which has 10,032  trainable parameters, excluding the number in the final layer for classification. The tasks have varying numbers of classes to be predicted, causing the classification layer to have varying numbers of parameters. CNN-1 has three convolutional layers, each one followed by ReLU and max pooling, the first two with 8 channels and the last one with 16. They are followed by a fully connected classification layer, using a softmax activation function. The first convolutional layer has a filter size of $7\times7$, and the other two have a filter size of $5\times5$. The convolutional layers have a stride of 1 and the max pooling layers have a stride of 2.\\
\indent We call the larger network CNN-2, with 116,214 parameters (not counting the classification layer). It is the same as CNN-1 except the convolutional layers have twice the number of channels, and a dense layer with 150 units is added before the classification layer. \\
\indent Note that the parameter configurations of both HiGSFA and CNNs have not been optimized for the best performance on the tasks below. They were designed to be lightweight according to general best practices \citep{hadji2018we} \citep{escalante2016improved}. This allows for more trials and tighter confidence bounds while achieving fair performance on the tasks.
\subsection{Evaluation on Omniglot}
Omniglot is a handwritten character data set consisting of 50 alphabets with 14 to 55 characters each, each character having 20 samples \citep{lake2015human}.  The alphabets vary from real alphabets, such as Greek, to fictional ones, such as Alienese (from the TV show “Futurama”). Each sample was drawn by a different person for this data set. It is typically split into 30 training alphabets, and 20 testing alphabets. Note that the training-testing split separates the alphabets; all samples originating from all characters from a given alphabet appear in either the training set or the test set but not both. This makes it a transfer learning task as the training and test data set samples drawn from separate distributions.  

In the original work using the data set, the methods were first trained on the 30 background alphabets, and then a 20 way one shot classification task was performed. Two samples are taken from each of 20 characters from random evaluation alphabets. One sample is placed in what we’ll call a probe set, and the other in a target set. The methods then try to find the corresponding sample in the target set that is the same character as any given sample in the probe set.


\begin{figure}[ht]
  %\vspace{-0.2cm}
  \centering
   {\resizebox*{0.4 \textwidth}{!}{\includegraphics
    {files/omniglotnice.png}}}
  \caption[Example: 16-way One Shot Classification]{\textbf{16-way One Shot Classification}. Symbols on the left are presented to the algorithm, one at a time, and the task is to find the same character from the symbols on the right.}
  \label{fig-16way}
 \end{figure}
 
 



In the vein of the original Omniglot task, we compare several models in three challenges. In all challenges, we do 16 way one shot classification using 1-nearest-neighbor (1-NN) under the Euclidean distance. The challenges differ in how the test set is related to the training set:
\subsubsection{Challenge 0} From 16 random characters used for training, we take two samples that the models were trained on. These samples are placed in two sets, the probe and target sets, such that each set contains one sample of each character. The model under consideration extracts features from each image. We then iterate through each feature vector from images in the probe set and find the closest feature vector from the target set. If those two vectors belong to images of the same class, then we count it as a success.

\subsubsection{Challenge 1} Same as above, but we take characters used during training for the probe set and perform classification on samples that were not used during the training.

\subsubsection{Challenge 2} Same again, but now we do the classification on characters that do not belong to alphabets used during training.

\subsection{Omniglot architectures}

 All model architectures are the same for MNIST and Omniglot, but the Omniglot images are resized to $35\times35$, having the effect that HiGSFA outputs 784 features. The number of model parameters does not change as the weights are shared for the image patches. The HiGSFA features used for classification are simply the 784 output features and we do not train a neural network classifier on them.

The total number of parameters in the CNNs depend on the number of training classes, due to the classification layer. We fix the number of alphabets to 8 and vary the number of characters per class to be 4, 6, 8, 10, 12 and vice versa. The number of parameters for CNN-1 range between 18k and 35k, and for CNN-2 range between 121k and 130. If we do not count the parameters from the final classification layer, then the number of parameters for CNN-1 for these tasks is always 10,032  and the number for CNN-2 is 116,214.

After training the CNNs, we perform feature extraction by intercepting the output of the second-to-last layer. Here the assumption is that CNNs learn a representation for the classification layer \citep{DBLP:journals/corr/RazavianASC14}. We are then interested in comparing the strength of HiGSFA and CNN representations when used by a 1-NN classifier.


\begin{table*}[ht]%[!ht]
\centering
\begin{tabular}{  r | l l | l l | l l}

%  \cline{1-7}
\hline
  Samples\,
 & HiGSFA & & CNN-1 && CNN-2 &\Tstrut  \\
         & Acc. & Std.    &  Acc.  & Std.  & Acc.  & Std.  \Bstrut     \\
%  \cline{1-7}   
\hline
    5\,     & 35.683    & $\pm$ 0.430  & $\textbf{72.361}$   &$\pm$ 0.365 & 72.320 &$\pm$ 0.094\,  \,\,\ \Tstrut\\
  10\,   & 75.736    &    $\pm$ 0.222  & $\textbf{80.392}$   &$\pm$ 0.241 & 79.551 &$\pm$ 0.175     \\
  50\,   & $\textbf{92.970}$    &$\pm$ 0.050  & 90.320   &$\pm$ 0.101   & 91.465 & $\pm$ 0.070    \\
  200\,  & $\textbf{96.246}$    &$\pm$ 0.027   & 94.672   &$\pm$ 0.062  & 95.648 & $\pm$ 0.051    \\
  500\,   & 97.188   &$\pm$ 0.013    & $96.579$   &$\pm$ 0.046  & \textbf{97.308} &$\pm$ 0.054  \\
  2000\,   & 97.887   &$\pm$ 0.009 & 98.247   &$\pm$ 0.020  & $\textbf{98.571}$ & $\pm$ 0.023   \\
  6000\,   & 98.134   & $\pm$ 0.008   & 98.687   &$\pm$ 0.014 & $\textbf{98.949}$ &$\pm$ 0.015  \\
\end{tabular}
\caption[Result: MNIST Accuracies]{\textbf{MNIST Accuracies.} The percentage of correctly classified samples on the test set along with the standard error of the mean (SEM). }
\label{tab:totalresults}
\end{table*} 



\subsection{Training}

The models were trained on varying amounts of samples per character. The HiGSFA network was trained to solve the optimization problem on each image patch, one layer at a time.  All neural networks were trained in Keras  \citep{chollet2015keras} using ADAM  \citep{kingma2014adam}, with default parameters, to minimize cross-entropy.\\ \indent After each epoch, the error was calculated on the validation set. Early stopping was performed after the validation error had increased four times in total during the training. The training for Omniglot is the same, except instead of early stopping, the CNNs were trained for 20 epochs in all cases.


\begin{figure*}[ht]%
    \centering{{\includegraphics[width=5.7cm]{files/index3a.png} }}%
    \qquad{{\includegraphics[width=5.7cm]{files/index6a.png} }}%
    \qquad{{\includegraphics[width=5.7cm]{files/index2a.png} }}%
    \qquad{{\includegraphics[width=5.7cm]{files/index5a.png} }}%
    \qquad{{\includegraphics[width=5.7cm]{files/index1a.png} }}%
    \qquad
    {{\includegraphics[width=5.7cm]{files/index4a.png} }}%
    \caption[Result: Classification Accuracies]{\textbf{Classification Accuracies}. There are either 8 alphabets and we vary the characters per alphabet, or vice versa. The error bars indicate the standard error of the mean. These plots are best viewed in color.}%
    \label{fig:plots}%
\end{figure*}



\section{Results}
\label{measuring_results}

\subsection{MNIST Results}
We trained the models using 5, 10, 50, 200, 2000 or 4000 samples per digit. In table \ref{tab:totalresults}, we see the statistics from 100 runs, where the models were trained from random initializations, evaluated and tested.  The convolutional networks have the highest accuracies when there are 2000 or more samples per class and when there are only 5 or 10 samples per class. \\ \indent However, HiGSFA has a higher accuracy than the CNN with a similar number of parameters for 500 samples per class. Furthermore, HiGSFA has higher accuracies than both CNNs for 200 and 50 samples per class. The CNN with a larger number of parameters always has higher prediction accuracies than the one with a lower number of parameters.

\subsection{Omniglot Results}

The 1-NN classifier uses the second-to-last CNN outputs or HiGSFA features. We fix either the number of alphabets, or characters-per-alphabet, to be 8 and vary the other number from 4 to 12 in increments of 2. The number of samples per character is either 4 or 16. The largest total number ($\text{alphabets} \times \text{characters per alphabet} \times \text{samples per character}$) of samples used for training is 1536 and the lowest is 128. \\
\indent In figure \ref{fig:plots}, we see the average of all the runs over the different samples per characters and number of classes. In all of the challenges, the CNNs have higher accuracies than HiGSFA. On average, CNN-2 has higher accuracies in challenges 0 and 2. Neither CNN achieves significantly better accuracy than the other in challenge 1. 



\section{Discussion and conclusion}
\label{measuring_discussion}


\noindent The work of this paper is intended to facilitate understanding of algorithms from the point of view of having particularly low numbers of samples. We present simple-to-implement challenges that allow for evaluation of data efficiency in the context of representation learning. \\
\indent For the models experimented on, we see that the CNNs usually perform better, but HiGSFA outperforms the CNNs on 50 and 200 sample training sets from the MNIST data. One can speculate that the default CNN architectures ensure generalization through max-pooling whereas SFA mostly learns to generalize from a moderately sized data set. \\
\indent Another explanation for the different ranges of comparative performance optima is the choice of delta-threshold of HiGSFA. The method overestimates the slowness of the slowest features when it has too few samples. This has the effect that fewer PCA features are selected for a lower number of samples. On the other hand, with more than 200 samples, there could be too many PCA features chosen. Setting the number of slow features to be a constant for all sample sizes could be better for robustness than fixing the delta threshold. \\
\indent Notice the trend in challenge 0: the accuracy goes down as the number of samples increases. This is due to the samples used for the probe and target sets being drawn from the training set and we are training and testing on larger sets as we move from left to right. \\
\indent Overall, for the Omniglot challenges, the accuracies of the CNNs lie comfortably above the HiGSFA accuracies, but it’s not always discernible whether the larger or the smaller CNN performs better. An explanation for this could be that the tasks are not difficult enough for more parameters to be necessary.  The local optimality of GSFA could result in an insufficiently robust or transferable representation if there are many classes and few samples per class. \\ 
\indent These challenges are more complicated set of classification tasks than the MNIST ones, with a larger number of classes overall. This give CNNs an opportunity to take advantage of having been trained directly for classification when they are presented a similar task. Although HiGSFA takes advantage of class labels, it suffers in comparison for not taking into account the downstream task during training.\\
\indent For future work, a complete extension of the experiments here could include an analysis on the effect that different type of data would have on the performance. This would yield further insight than varying the number of rather homogeneous data used for training. Additionally, the performance of a wider array of popular methods can be compared. \\
\indent More types of benchmarks for comparing different models over varying training set sizes would be helpful for this kind of research. Knowledge gained from them would as well allow practitioners to choose the right model for the scale and type of the problem they wish to solve.  These experiments give rise to the question: how can these methods with their different strengths and weaknesses profit from each other?



